Automatic Detection of Webpages that Share the Same Web Template

Template extraction is the process of isolating the template of a given webpage. It is widely used in several disciplines, including webpages development, content extraction, block detection, and webpages indexing. One of the main goals of template extraction is identifying a set of webpages with the same template without having to load and analyze too many webpages prior to identifying the template. This work introduces a new technique to automatically discover a reduced set of webpages in a website that implement the template. This set is computed with an hyperlink analysis that computes a very small set with a high level of confidence.

==> eptcsdata.tex <==
\providecommand{\firstpage}{2}
\providecommand{\publicationstatus}{M.H. ter Beek and A. Ravara (Eds.): 10th International Workshop on\\ Automated Specification and Verification of Web Systems (WWV'14) \\
EPTCS 163, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.163.2}{10.4204/EPTCS.163.2}}
\pdfoutput=1

